Moduli Spaces of Lagrangian Surfaces in $\mathbb{CP}^2$ obtained from Triple Grid Diagrams

Links in $S^3$ as well as Legendrian links in the standard tight contact structure on $S^3$ can be encoded by grid diagrams. These consist of a collection of points on a toroidal grid, connected by vertical and horizontal edges. Blackwell, Gay and second author studied triple grid diagrams, a generalization where the points are connected by vertical, horizontal and diagonal edges. In certain cases, these determine Lagrangian surfaces in $\mathbb{CP}^2$. However, it was difficult to construct explicit examples of triple grid diagrams, either by an approximation method or combinatorial search. We give an elegant geometric construction that produces the moduli space of all triple grid diagrams. By conditioning on the abstract graph underlying the triple grid diagram, as opposed to the grid size, the problem reduces to linear algebra and can be solved quickly in polynomial time.

==> blah.tex <==
\begin{comment}
\section{Method to get Triple Grid Diagrams from Tait-coloured cubic graphs}


\begin{theorem}
For every Tait-coloured abstract bipartite cubic graph, there exists a Triple Grid diagram.
\end{theorem}

We will first get coordinate representations of corresponding Triple Grids which we will then convert to combinatorial Triple Grid diagrams.

\begin{defn}
The coordinate representation of a Triple Grid consists of $2n$ points(vertices/dots) in $\mathbb{T}^2 = \mathbb{R}^2/\mathb{Z}^2$, where $n$ is a positive integer. These points $(x_i,y_i,z_i)_1^{2n}$ satisfy the following conditions:
\begin{itemize}
    \item For each $x \in \mathbb{I}$, either there are strictly two points which have $x$ as their x coordinate, or none. 
    \item For each $y \in \mathbb{I}$, either there are strictly two points which have $y$ as their y coordinate, or none. 
    \item For each $z \in \mathbb{I}$, either there are strictly two points which have $z$ as their z coordinate, or none. 
    \item The coordinates of a point satisfy the equation $x + y + z = 0$. 
\end{itemize}
\end{defn}

\textcolor{blue}{ Are we defining diagonals as positive-sloped or negative-sloped?}
\textcolor{blue}{Do we want to loosen the definition for when edges collapse/overlap?}

\subsection{Combinatorial Method}

Let $G = (V, E)$ be a cubic (tri-valent) graph that is Tait-coloured such that $|V| = 2n$. By definition of Tait-colouring, $E = E_{red} \cup E_{blue} \cup E_{green}$ such that for each vertex $v_i \in V$, the colors of the incident edges are different. We follow the following steps to get the corresponding Triple Grid diagrams. 

\renewcommand{\labelitemi}{\blacksquare}
\begin{itemize}
    \item The vertices in the graph correspond to the dots in the Triple Grid Diagram. For each vertex $v_i \in V$, assign co-ordinates $(x_i,y_i,z_i)$ such that $z_i = x_i - y_i$. ($2n$ equations)
    \item For each edge $e_{(i,j)} \in E_{red}$, set $y_i = y_j$. The red edges in the graph correspond to the red horizontal arcs of the triple grid diagram. ($n$ equations)
    \item Similarly, for each edge $e_{(i,j)} \in E_{blue}$, set $y_i = y_j $. The blue edges in the graph correspond to the blue vertical arcs of the triple grid diagram. ($n$ equations)
    \item For each edge $e_{(i,j)} \in E_{green}$, set $ z_i = z_j  \bmod \mathbb{Z}$. The green  edges in the graph correspond to the green diagonal arcs of the triple grid diagram. ($n$ equations)    
\end{itemize}

 A solution to the above equations corresponds to a coordinate representation of a triple grid diagram.

 \subsection{Geometric Method}

 Let $\Gamma$ be an abstract Tait-coloured cubic graph.  

\section{The moduli space of Triple Grid Diagrams for a Cubic Tait-Coloured Graph}

We started with a Cubic Tait-Coloured graph $G = (V,E)$ such that $|V|=2n$ and got Triple Grid Diagrams of size $n$ by solving a system of linearly independent equations. We start with $6n$ variables corresponding to the (x,y,z) coordinates of each of the $2n$ points (vertices) and we solve $5n$ linearly independent equations coming from the steps in the method outlines in the previous section. So we have a solution space with at least $n$ dimensions.

Also note that since these points are on a torus, we are actually working in $\mathbb{R} \mod \mathbb{Z}$. So we can fix the coordinates of one of the vertices as $(0,0,0)$, reducing the dimensions of the solution space by $2$. 

Hence for a cubic Tait-coloured graph with $2n$ vertices, we get a solution space of $d$ dimensions, where $d>n-2$. 

\begin{eg}[$K_{3,3}$]
[Insert Digram of $K_{3,3}$]

`\begin{itemize}
    \item The vertices in the graph correspond to the dots in the Triple Grid Diagram. Let $X_j \in K_{3,3}$ have coordinates $(x_j,y_j,z_j)$ and let $O_j \in K_{3,3}$ have coordinates $(x_{3+j},y_{3+j},z_{3+j})$. Here $z_i = x_i- y_i$ for all $v_i \in V$.
    \item Looking at the red edges, $X_1$ is connected to $O_2$. So $x_1 = x_{3+2} = x_5$. Similarly, we get $x_2 = x_6$ and $x_3 = x_4$. 
    \item Next, looking at the blue edges, we get $y_1 = y_4$, $y_2 = y_5$, and $y_3 = y_6$.
    \item Finally, looking at the green edges, we get $z_1 = z_6$,$z_2 = z_4$, and $z_3 = z_5$.  
\end{itemize}

Solving these equations, we get the following basis for the solution space.


\end{eg}


The possible moves on this Triple Grid Diagram are :

\begin{itemize}
    \item Crossing Change: When we cross a Type 1 hypersurface.
    \item Commutation Move: When we cross a Type 2 hypersurface.    
\end{itemize}

\begin{claim}
The number of regions in the moduli space is at max $(n-1)!$. 
\end{claim}

\textcolor{red}{How many Type 1 and how many Type 2 hypersurfaces are there?}  

\end{comment}

\begin{comment}
\begin{figure}[htpb]
    \centering
    \includesvg[pretex=\tiny\sffamily]{figures/K_3,3.svg}
    \caption{Broken svg}
    \label{fig:Broken}
\end{figure}
\end{comment}
